Numerical Computations for Backward Doubly SDEs and SPDEs

In this paper we present two numerical schemes of approximating solutions of backward doubly stochastic differential equations (BDSDEs for short). We give a method to discretize a BDSDE. And we also give the proof of the convergence of these two kinds of solutions for BDSDEs respectively. We give a sample of computation of BDSDEs.

==> setup/Ccode.tex <==
%\lstloadlanguages{C, C++, csh, make,fortran,R,matlab}
\lstloadlanguages{C, C++}
\lstset{language=C++,
    tabsize=4,
    keepspaces=true,
    breakindent=22pt,
    numbers=left,
    stepnumber=1,
    numberstyle=\tiny,
    basicstyle=\footnotesize\ttfamily,
    showspaces=false,
    flexiblecolumns=true,
    breaklines=true,
    breakautoindent=true,
    breakindent=4em,
    escapeinside={/*@}{@*/},
    frame=single,
}

\lstset{
    commentstyle=\color[rgb]{0.133,0.545,0.133}\textsl,
    keywordstyle=\color{blue},
    caption=\lstname,
    breaklines=true,
    columns=flexible,
    mathescape=true
    xleftmargin=3em,
    xrightmargin=1em,
}

\lstdefinestyle{numbers}{numbers=left,
    stepnumber=1,
    numberstyle=\small,
    numbersep=1em
}


==> setup/Rcode.tex <==
\lstloadlanguages{R}

\lstdefinelanguage{Renhanced}[]{R}{%
  morekeywords={acf,ar,arima,arima.sim,colMeans,colSums,is.na,is.null,%
  mapply,ms,na.rm,nlmin,replicate,row.names,rowMeans,rowSums,seasonal,%
  sys.time,system.time,ts.plot,which.max,which.min},
%  deletekeywords={c},
  alsoletter={.\%},%
  alsoother={:_\$}
}

\lstset{language=Renhanced,
    caption=\lstname,
    extendedchars=true,
    basicstyle=\small\ttfamily,
    keywordstyle=\color[rgb]{0,0,1},                    % keywords
    basicstyle=\footnotesize\ttfamily,
    frame=single,
%    columns=fixed
    columns=flexible,
    numbers=left,
    showspaces=false,
    stepnumber=1,
    numbersep=5pt,
    numberstyle=\tiny,
    commentstyle=\color[rgb]{0.133,0.545,0.133}\textsl,    % comments
    showstringspaces=false,
    index=[1][keywords],
    indexstyle=\indexfonction,
    mathescape=false,
}

\newcommand{\indexfonction}[1]{\index{#1@\texttt{#1}}}


==> setup/cnthm.tex <==
\newtheorem{theorem}{定理\ }[section]
\newtheorem{thm}[theorem]{定理\ }
\theoremstyle{definition}
\newtheorem{corol}[theorem]{推论\ }
\newtheorem{Def}[theorem]{定义\ }
\newtheorem{definition}[theorem]{定义\ }
\newtheorem{example}[theorem]{例\ }
\newtheorem{hypo}[theorem]{假设\ }
\newtheorem{lemma}[theorem]{引理\ }
\newtheorem{prop}[theorem]{命题\ }
\newtheorem{proposition}[theorem]{命题\ }
\newtheorem{remark}[theorem]{注\ }
\newtheorem{exercise}[theorem]{练习\ }
\newtheorem{thinking}[theorem]{思考\ }
\newtheorem{problem}[theorem]{问题\ }
\newtheorem{homework}[theorem]{作业\ }
%\newenvironment{proof}[1][Proof]{\noindent\textbf{#1.} }{\ \rule{0.5em}{0.5em}}
\renewenvironment{proof}[1][证明]{\noindent\textbf{#1.} }{}
%\hfill $\square$


==> setup/fcode.tex <==
%\lstloadlanguages{C, C++, csh, make,fortran,R,matlab}
\lstloadlanguages{C, C++}
\lstset{language=fortran,
    tabsize=4,
    keepspaces=true,
    breakindent=22pt,
    numbers=left,
    stepnumber=1,
    numberstyle=\tiny,
    basicstyle=\footnotesize\ttfamily,
    showspaces=false,
    flexiblecolumns=true,
    breaklines=true,
    breakautoindent=true,
    breakindent=4em,
%    escapeinside={/*@}{@*/},
    frame=single,
}

\lstset{
    commentstyle=\color[rgb]{0.133,0.545,0.133}\textsl,
    keywordstyle=\color{blue},
    caption=\lstname,
    breaklines=true,
    columns=flexible,
    mathescape=true
    xleftmargin=3em,
    xrightmargin=1em,
    mathescape=false,
%    escapechar=?                            % escape to latex with ?..?
%    upquote=true,                                                % upright quotes
}

\lstdefinestyle{numbers}{numbers=left,
    stepnumber=1,
    numberstyle=\small,
    numbersep=1em
}


==> setup/mcode.tex <==
\lstloadlanguages{matlab}

\lstdefinelanguage{matlabfloz}[]{matlab}{%
    alsoletter={...},%
    morekeywords={%                                             % keywords
    break,case,catch,continue,elseif,else,end,for,function,global,%
    if,otherwise,persistent,return,switch,try,while,...},%
    comment=[l]\%,%                                             % comments
    morecomment=[l]...,%                                     % comments
    morestring=[m]',%                                           % strings
}[keywords,comments,strings]%

\lstset{%
%    basicstyle={\lstbasicfont\footnotesize},        % use font and smaller size
    basicstyle=\footnotesize\ttfamily,
    showstringspaces=false,                                % do not emphasize spaces in strings
    tabsize=4,                                                    % number of spaces of a TAB
    mathescape=true,escapechar=?                            % escape to latex with ?..?
    upquote=true,                                                % upright quotes
    aboveskip={1.5\baselineskip},                            % a bit of space above
    columns=fixed,                                                % nice spacing
    breaklines=true,
    breakautoindent=true,
    breakindent=4em,
%    escapeinside={/*@}{@*/},
    %
    % the following is for replacing some matlab relations like >= or ~=
    % by the corresponding LaTeX symbols, which are much easier to read ...
%    literate=%
%        {~}{{$\neg$}}1 %                \neg
%        {<=}{{\tiny$\leq$}}1 %        \leq
%        {>=}{{\tiny$\geq$}}1 %        \geq
%        {~=}{{\tiny$\neq$}}1 %        \neq
%        {delta}{{\tiny$\Delta$}}1% \Delta
}


\lstset{
    language=matlab,
    frame=single,
%    basicstyle=\ttfamily,
%    keywordstyle=\bfseries,
%    columns=fixed
    numbers=left,
%    showspaces=true,
    stepnumber=1,
    numbersep=5pt,
    numberstyle=\tiny,
    keywordstyle=\color[rgb]{0,0,1},                    % keywords
    commentstyle=\color[rgb]{0.133,0.545,0.133},    % comments
    stringstyle=\color[rgb]{0.627,0.126,0.941},  % strings
}

%\usepackage{moreverb}  % \listinginput[1]{1}{code/helloworld.f}

%\listinginput[n]{m}{filename}
%where
%n = increment: a line number will appear every n lines
%m = first line to be numbered


==> setup/setup.tex <==
\setcounter{MaxMatrixCols}{50}


%\textwidth 148mm
%\textheight 220mm
%\headheight=1.5\ccht
%\headsep=15pt
%\topmargin=5mm
%\oddsidemargin=6mm
%\evensidemargin=6mm
%\raggedbottom

\textwidth 156mm
\textheight 230mm
%\headheight=1.5\ccht
\headsep=15pt
\topmargin=5mm
\oddsidemargin=5mm
\evensidemargin=5mm
%\setlength{\oddsidemargin}{5mm}
%\setlength{\evensidemargin}{5mm}
%\raggedbottom
\flushbottom



%\numberwithin{equation}{section} % class book doesn't need the command

%\vfuzz2pt % Don't report over-full v-boxes if over-edge is small
%\hfuzz2pt % Don't report over-full h-boxes if over-edge is small


==> setup/zihao.tex <==
\newcommand{\chuhao}{\fontsize{42pt}{\baselineskip}\selectfont}
\newcommand{\xiaochuhao}{\fontsize{36pt}{\baselineskip}\selectfont}
\newcommand{\yihao}{\fontsize{28pt}{\baselineskip}\selectfont}
\newcommand{\erhao}{\fontsize{21pt}{\baselineskip}\selectfont}
\newcommand{\xiaoerhao}{\fontsize{18pt}{\baselineskip}\selectfont}
\newcommand{\sanhao}{\fontsize{15.75pt}{\baselineskip}\selectfont}
\newcommand{\sihao}{\fontsize{14pt}{\baselineskip}\selectfont}
\newcommand{\xiaosihao}{\fontsize{12pt}{\baselineskip}\selectfont}
\newcommand{\wuhao}{\fontsize{10.5pt}{\baselineskip}\selectfont}
\newcommand{\xiaowuhao}{\fontsize{9pt}{\baselineskip}\selectfont}
\newcommand{\liuhao}{\fontsize{7.875pt}{\baselineskip}\selectfont}
\newcommand{\qihao}{\fontsize{5.25pt}{\baselineskip}\selectfont}

